Genius: A Generalizable and Purely Unsupervised Self-Training Framework For Advanced Reasoning

Advancing LLM reasoning skills has captivated wide interest. However, current post-training techniques rely heavily on supervisory signals, such as outcome supervision or auxiliary reward models, which face the problem of scalability and high annotation costs. This motivates us to enhance LLM reasoning without the need for external supervision. We introduce a generalizable and purely unsupervised self-training framework, named Genius. Without external auxiliary, Genius requires to seek the optimal response sequence in a stepwise manner and optimize the LLM. To explore the potential steps and exploit the optimal ones, Genius introduces a stepwise foresight re-sampling strategy to sample and estimate the step value by simulating future outcomes. Further, we recognize that the unsupervised setting inevitably induces the intrinsic noise and uncertainty. To provide a robust optimization, we propose an advantage-calibrated optimization (ACO) loss function to mitigate estimation inconsistencies. Combining these techniques together, Genius provides an advanced initial step towards self-improve LLM reasoning with general queries and without supervision, revolutionizing reasoning scaling laws given the vast availability of general queries. The code will be released at https://github.com/xufangzhi/Genius.

==> sections/1.introduction.tex <==
\section{Introduction}

Reasoning skills are among the key foundational capabilities for Large Language Models (LLMs)~\cite{achiam2023gpt, team2023gemini}.
% Large Language Models (LLMs)~\cite{achiam2023gpt, team2023gemini} have demonstrated remarkable performances in reasoning-intensive tasks with large-scale training on well-annotated data.
Prior endeavors~\cite{qwq-32b-preview} have advanced LLM reasoning through large-scale post-training on well-annotated data.
However, acquiring high-quality in-domain reasoning data remains challenging, involving extensive human efforts and huge time costs. \changh{The motivation not detailed enough, maybe introduce it this way:}\chang{Reasoning skills are crucial for LLMs to achieve human-level intelligence. Current work found out in addition to pretraining, it is also essential to inject reasoning ability at the post training stage. To achieve this, previous methods often rely on supervision: 1) verification of answers 2) reward models. Reward models are not reliable, difficult to train and generalize, and have reward hacking problems.Verifiers limit the scope of data. Even best models like R1 are limited by these problems, which could affect scaling of reasoning models. It would revolutionize reasoning scaling law if we could achieve effective and efficient improvement in reasoning post training through general data.}

\chang{These limitations raise a research question: Could we incorporate annotation-free scalable general data for improving reasoning abilities of LLM ?}

\changh{!!!\#1}\chang{We tackle this problem by proposing a novel post-training framework, named Genius, ..., surprisingly after training xxx steps on xxx data, could xxx improve reasoning performance. Inspried by} recent efforts on \emph{self-play} techniques~\cite{tao2024survey,zhang2024survey}, our algorithm largely consists of three steps: (1) synthesizing response $a$ based on the given query $x$, (2) rewarding the response data $a$, and (3) optimizing itself using the curated data.\changh{I feel introducing a self-play framework here, which is part of prior work is somehow limiting the scope. }



\changh{merge this paragraph into the first paragraph. dont talk about self-play, only discusses motivation about annotation \& scaling of data sources}Notable progress has been made in applying such \emph{self-play} methods to improve specific reasoning abilities (e.g., mathematics).
% These works either rely on the output supervision as the reward signal~\cite{trung2024reft,xu2024interactive}, or 
These early endeavors utilize in-domain reasoning data and rely on either explicit outcome supervision (Fig.~\ref{intro}(a)) ~\cite{trung2024reft,cheng2024vision} or a reward model to give supervision signals (Fig.~\ref{intro}(b))~\cite{jiao2024learning}.
Yet, not all reasoning problems yield extractable solutions and explicit ground-truth. Extending these self-play techniques to broader reasoning domains proves to be intractable.
Also, the training of a generalized reward model is hindered by the availability of large-scale supervised data.
Therefore, we delve into a more challenging but promising direction to \emph{self-improve LLM reasoning ability \textbf{without both in-domain supervised data and external auxiliary}} (Fig.~\ref{intro}(c)). 

\begin{figure}[t]
\large
\centering
\includegraphics[scale=0.7]{Figures/Intro.pdf}
\caption{Different paradigms to boost LLM reasoning. (a) and (b) abstract previous methods, which require supervision. (c) depicts the ultimate goal of our research.}
\label{intro}
\vspace{-1em}
\end{figure}

\changh{!!!\#2}Firstly, it is non-trivial to address \emph{how to sample and reward the LLM responses without external auxiliary.}
One intuitive solution is to roll out the whole reasoning path with the LLM itself, and then evaluate the response based on the confidence of the sequence~\cite{xu2024interactive}, or by re-prompting it to assign scores~\cite{yuanself} or resorting to the self-consistency~\cite{prasad2024self}.
However, these attempts primarily concentrate on instance-level rewards.
Recent efforts like~\cite{zhang2024chain} employ step-level self-exploration and exploitation, 
but they naturally inherit the myopic limitation of auto-regressive generation~\cite{ma2024non}.
Additionally, some search-based works (e.g., MCTS-style methods) require intricate backtracking processes, incurring significantly high costs in training time.

\changh{!!!\#3}Secondly, it remains an open question on \emph{how to improve the robustness of the self-play framework during the optimization?}
It is inevitable to induce noise when using self-rewarding to select preference pairs.
That is, a higher level of model confidence does not necessarily result in a better response.
Previous self-play methods simply employ either supervised fine-tuning~\cite{zelikman2022star} or reinforced learning strategies~\cite{yuanself} for optimization, which neglects the uncertainty of self-supervision. 
While some works attempt to offer robust solutions~\cite{liang2024robust},
these general optimization strategies overlook incorporating feedback from the sampling and self-rewarding process, leading to suboptimal outcomes.

\changh{merge this part into the symbol !!!\#1, tell people you've magically solved the RQ }This work proposes a novel self-play framework, named \ours, to boost the LLM reasoning ability \textbf{without reliance on external reward models and in-domain data}.
\changh{merge this part into the symbol !!!\#2, tell people how you solved the external auxillary. }To address the limitations of auto-regressive generation,
we sample multiple candidates for the next step and assess their respective values through foresight.
The model confidence of the foresight paths creates a distribution,
which can be sampled to determine the next steps (\emph{exploration}) and resampled to construct step-level preference pairs (\emph{exploitation}).
Incorporating the foresight confidence, \ours also dynamically updates the step value and calculates the advantage of each selected step.
\changh{merge this part into the symbol !!!\#3, tell people how you solved the not robust optimization. }To overcome the limitations of previous optimization methods, we design an advantage-calibrated loss function to punish the inconsistent estimation between foresight confidence and step advantage.
Extensive experiments on diverse reasoning benchmarks verify the superiority of \ours to self-play from general queries. Without any external supervision, \ours improves the LLaMA3.1-8B reasoning performance by nearly 8\%.
Follow-up ablation and analysis experiments also provide in-depth insights.

The major contributions of our work are:
\changh{Generally, I feel that only the first contribution is exciting, and the other two quite plain. Perhaps contributions are not a optimal way to end an exciting paper. Discussing about future implications might be more exciting.}

\noindent (1) \textbf{A generalizable and purely unsupervised self-play framework \ours:} 
Different from previous self-play paradigms, \ours can effectively boost LLM reasoning capability simply from general instructions in a purely unsupervised manner. 

\noindent (2) \textbf{Major technical contributions:} 
To address the LLM myopic sampling and unreliable self-rewarding,
we provide a step-wise re-sampling strategy via foresight rewarding.
Based on it,
we design an advantage-calibrated loss function for robust optimization.
\changh{this point seems a bit strange... normally emphasizing your method is new seems like you don't have much exciting discoveries }
% \noindent (2) \textbf{Step-level sampling via foresight rewarding and advantage-calibrated loss design.}

\noindent (3) \textbf{Extensive evaluations and superior performances.} 
\ours boosts base LLM by almost 8\% across various reasoning benchmarks, requiring merely 25K general instructions. Extensive analysis verifies the effectiveness of each module and provides valuable insights.


\changh{perhaps add a paragraph to emphasize future implications} \chang{Our findings illustrate a unique perspective on improving LLM reasoning abilities -- LLM itself contains the ability to enhance its reasoning ability without any forms of supervision. We reveal that scaling law on general data consistently improves with more training steps (cite results in \S 5.3), and considering the vastness of general data, the scaling would be very helpful for improving reasoning.}

